A Systematic Exploration of Kilonova Candidates from Neutron Star Mergers During the Third Gravitational Wave Observing Run

We present a comprehensive analysis of 653 optical candidate counterparts reported during the third gravitational wave (GW) observing run. Our sample concentrates on candidates from the 15 events (published in GWTC-2, GWTC-3 or not retracted on GraceDB) that had a >1% chance of including a neutron star in order to assess their viability as true kilonovae. In particular, we leverage tools available in real time, including pre-merger detections and cross-matching with catalogs (i.e. point source, variable star, quasar and host galaxy redshift datasets), to eliminate 65% of candidates in our sample. We further employ spectroscopic classifications, late-time detections and light curve behavior analyses, and conclude that 66 candidates remain viable kilonovae. These candidates lack sufficient information to determine their classifications, and the majority would require luminosities greater than that of AT2017gfo. Pre-merger detections in public photometric survey data and comparison of catalogued host galaxy redshifts with the GW event distances are critical to incorporate into vetting procedures, as these tools eliminated >20% and >30% of candidates, respectively. We expect that such tools which leverage archival information will significantly reduce the strain on spectroscopic and photometric follow-up resources in future observing runs. Finally, we discuss the critical role prompt updates from GW astronomers to the EM community play in reducing the number of candidates requiring vetting.

==> abstract1.tex <==
Talk Title: Needles in the Haystack: Optimizing Searches for Kilonovae
The discovery of GW170817 and GRB\,170817A in tandem with transient AT\,2017gfo cemented the connection between neutron star mergers, short gamma-ray bursts (GRBs), and kilonovae. Since then, efforts to follow-up short GRBs and GW events have unearthed little proof of another definitive kilonova. In this talk, I will discuss our efforts to probe the diversity and detectability of kilonovae using existing observations of both short GRBs and graviational waves (GWs). I will first present a comprehensive catalog containing optical and near-infrared follow-up of 85 short GRBs, and discuss the diversity of kilonovae that it reveals. Next, I will introduce our analysis of over 650 candidate kilonova counterparts to 17 merger events from the third GW observing run. I will conclude by making recommendations for efficient follow-up of future nearby short GRBs and GW events.

%%% SGRB paper
The discovery of GW170817 and GRB\,170817A in tandem with AT\,2017gfo cemented the connection between neutron star mergers, short gamma-ray bursts (GRBs), and kilonovae. To investigate short GRB observations in the context of diverse kilonova behavior, we present a comprehensive optical and near-infrared catalog of 85 bursts discovered over 2005--2020 on timescales of $\lesssim12$~days. The sample includes previously unpublished observations of 23 bursts, and encompasses both detections and deep upper limits. We identify 11.8\% and 15.3\% of short GRBs in our catalog with upper limits that probe luminosities lower than those of AT~2017gfo and a fiducial NSBH kilonovae model (for pole-on orientations), respectively. We quantify the ejecta masses allowed by the deepest limits in our catalog, constraining blue and `extremely blue' kilonova components of 14.1\% of bursts to $M_{\rm ej}\lesssim0.01-0.1 M_{\odot}$. The sample of short GRBs is not particularly constraining for red kilonova components. Motivated by the large catalog as well as model predictions of diverse kilonova behavior, we investigate modified search strategies for future follow-up to short GRBs. We find that ground-based optical and NIR observations on timescales of $\gtrsim 2$~days can play a significant role in constraining more diverse outcomes. We expect future short GRB follow up efforts, such as from the {\it James Webb Space Telescope}, to expand the reach of kilonova detectability to redshifts of $z\approx 1$.

%%% O3 Candidates Paper
In 2017, the serendipitous detection of GW170817, GRB\,170817 and kilonova AT2017gfo opened the doors for a new era of multimessenger astronomy. Though it delivered other exciting discoveries, the third gravitational wave (GW) observing run (O3) failed to produce another secure electromagnetic (EM) counterpart to a GW-detected compact merger. EM follow-up efforts reported hundreds of kilonova candidates, a function of the 1,000+ degree$^2$ localizations and large GW-inferred distances of most events of interest. We present a comprehensive analysis of 666 candidate counterparts of 17 O3 events with a $>$1\% chance of being a BNS or NSBH or $>$10\% chance MassGap event. We employ tools available in real-time to determine which candidates could have been eliminated as kilonovae immediately, and find $>$50\% of GCN-reported follow-up efforts could have been conserved. Further, we use all available information to determine how many viable kilonova candidates remain and analyze their characteristics. We conclude by making recommendations for efficient EM follow-up in the fourth GW observing run.
